Unbiased Watermark for Large Language Models

The recent advancements in large language models (LLMs) have sparked a growing apprehension regarding the potential misuse. One approach to mitigating this risk is to incorporate watermarking techniques into LLMs, allowing for the tracking and attribution of model outputs. This study examines a crucial aspect of watermarking: how significantly watermarks impact the quality of model-generated outputs. Previous studies have suggested a trade-off between watermark strength and output quality. However, our research demonstrates that it is possible to integrate watermarks without affecting the output probability distribution with appropriate implementation. We refer to this type of watermark as an unbiased watermark. This has significant implications for the use of LLMs, as it becomes impossible for users to discern whether a service provider has incorporated watermarks or not. Furthermore, the presence of watermarks does not compromise the performance of the model in downstream tasks, ensuring that the overall utility of the language model is preserved. Our findings contribute to the ongoing discussion around responsible AI development, suggesting that unbiased watermarks can serve as an effective means of tracking and attributing model outputs without sacrificing output quality.

==> content/sections/experiment.tex <==
\input{content/pieces/performance_table}
\input{content/pieces/violinplot}

\section{Experiments}\label{se:experiment}

We evaluate the performance of our Unbiased Watermarks on two important applications of seq2seq models: text summarization~(TS) and machine translation~(MT). 

\textbf{Machine Translation.} In the MT task, we apply the WMT'14 English~(En) to Romanian~(Ro) dataset, which contains 2,000 En-Ro pairs.
As for the model, we adopt the Multilingual Bart~(MBart) model~\cite{mbart}, and the official tokenizer of it.\footnote{\url{https://huggingface.co/facebook/mbart-large-en-ro}}

\textbf{Text Summarization.} In the TS task, we adopt the CNN-DM~\cite{cnn-dm} corpus and select 30,000 pairs to evaluate. The model applied is BART-large, which has 400M parameters.

\textbf{Metric.} The generation quality of the translations is evaluated based on BLEU score~\cite{papineni2002bleu}, which primarily emphasizes the lexical similarity, while the summarization is evaluated by ROUGE score~\cite{lin2004rouge}, which measures the overlap in terms of n-grams to assess the effectiveness of the summary in capturing the essential content from the reference summaries. BERTScore and Perplexity scores are included in both tasks as metrics to evaluate how well LLMs predict a sequence of words and the level of uncertainty or surprise the model has in making accurate predictions, respectively. 


\textbf{Baseline.} We compare $\delta$-reweight and $\gamma$-reweight with Soft Red List method proposed by \citet{kirchenbauer2023watermark}.

\textbf{Results.}





\subsection{Watermark detection}
\input{content/pieces/completion_demo_table}
\input{content/pieces/score_per_token}
